Movie101v2: Improved Movie Narration Benchmark

Automatic movie narration aims to generate video-aligned plot descriptions to assist visually impaired audiences. Unlike standard video captioning, it involves not only describing key visual details but also inferring plots that unfold across multiple movie shots, presenting distinct and complex challenges. To advance this field, we introduce Movie101v2, a large-scale, bilingual dataset with enhanced data quality specifically designed for movie narration. Revisiting the task, we propose breaking down the ultimate goal of automatic movie narration into three progressive stages, offering a clear roadmap with corresponding evaluation metrics. Based on our new benchmark, we baseline a range of large vision-language models, including GPT-4V, and conduct an in-depth analysis of the challenges in narration generation. Our findings highlight that achieving applicable movie narration generation is a fascinating goal that requires significant research.

==> figures/lexical-epoch.tex <==
\begin{figure}[t]
    \begin{center}
        \includegraphics[width=0.85\linewidth]{figures/assets/lexical-epoch.pdf}
    \end{center}
    \vspace{-8pt}
\caption{Lexical diversity of different datasets (dotted lines) and narrations generated by VideoChat-2 after fine-tuning on Movie101v2 (solid line). Movie101v2 represents its English version for lexical diversity comparison.}
\label{fig:lexical-epoch}
% \vspace{-8pt}
\end{figure}

==> figures/qualitative.tex <==
\begin{figure}[t]
    \begin{center}
        \includegraphics[width=1\linewidth]{figures/assets/qualitative.pdf}
    \end{center}
    \vspace{-8pt}
\caption{Qualitative results from our baseline models. Models show promise in recognizing environments, characters, and events. GPT-4V predictions offer rich details but are often prone to hallucinations. All models still fall short of the ground-truth narrations created by human experts.}
\label{fig:qualitative}
\vspace{-8pt}
\end{figure}

==> tables/linguistic.tex <==
\begin{table}[t]
\caption{\label{tab:linguistic-stat}
Linguistic Statistics.
}
\centering
\small
\begin{tabular}{@{}l|cccc|c@{}}
\toprule
 & Lexical & 2-gram & 3-gram & 4-gram & Perplexity\\ \midrule
VideoChatGPT & 4.3 & 28.2 & 57.7 & 76.5 & 33.4 \\
LLaVA Instruction & 9.6 & 48.7 & 79.9 & 92.9 & 39.4 \\
LLaVA Detail & 6.1 & 32.7 & 61.6 & 80.8 & 20.2 \\ \midrule
\textbf{Movie101v2-en} & \textbf{15.9} & \textbf{59.3} & \textbf{88.0} & \textbf{96.8} & \textbf{62.5} \\ \bottomrule
\end{tabular}
\end{table}

==> tables/main-results.tex <==
\begin{table*}[t]
\caption{\label{tab:main-res}
Model performance on Movie101v2. All scores are rescaled to a range of 0-100.
}
\vspace{-4pt}
\centering
\small
\begin{tabular}{@{}l|c|cccc|cccc@{}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Char.} & \multicolumn{4}{c|}{Movie101v2-zh} & \multicolumn{4}{c}{Movie101v2-en} \\ \cmidrule(l){3-10} 
 &  & L1-Env & L1-Char & \textbf{L1-Score} & \textbf{L2-Score} & L1-Env & L1-Char & \textbf{L1-Score} & \textbf{L2-Score} \\ \midrule
\multirow{2}{*}{VideoChat-2~\cite{videochat-2}} &  & 22.5 & 25.6 & 24.0 & 24.0 & 10.6 & 26.2 & 18.4 & 30.6 \\
 & \checkmark & 24.0 & 30.2 & 27.1 & 25.7 & 11.1 & 27.7 & 19.4 & 32.3 \\ \midrule
\multirow{2}{*}{Qwen-VL~\cite{qwen-vl}} &  & 31.2 & 34.9 & 33.0 & 27.9 & 15.1 & 27.6 & 21.4 & 29.5 \\
 & \checkmark & 34.0 & 39.7 & 36.8 & 31.5 & 16.9 & 30.3 & 23.6 & 32.0 \\ \midrule
GPT-4V & \checkmark & \textbf{50.0} & \textbf{53.0} & \textbf{51.5} & \textbf{37.4} & \textbf{37.1} & \textbf{43.3} & \textbf{40.2} & \textbf{38.9} \\ \bottomrule
\end{tabular}
\end{table*}
